Uncertainty-aware abstention in medical diagnosis based on medical texts

This study addresses the critical issue of reliability for AI-assisted medical diagnosis. We focus on the selection prediction approach that allows the diagnosis system to abstain from providing the decision if it is not confident in the diagnosis. Such selective prediction (or abstention) approaches are usually based on the modeling predictive uncertainty of machine learning models involved. This study explores uncertainty quantification in machine learning models for medical text analysis, addressing diverse tasks across multiple datasets. We focus on binary mortality prediction from textual data in MIMIC-III, multi-label medical code prediction using ICD-10 codes from MIMIC-IV, and multi-class classification with a private outpatient visits dataset. Additionally, we analyze mental health datasets targeting depression and anxiety detection, utilizing various text-based sources, such as essays, social media posts, and clinical descriptions. In addition to comparing uncertainty methods, we introduce HUQ-2, a new state-of-the-art method for enhancing reliability in selective prediction tasks. Our results provide a detailed comparison of uncertainty quantification methods. They demonstrate the effectiveness of HUQ-2 in capturing and evaluating uncertainty, paving the way for more reliable and interpretable applications in medical text analysis.

==> tables/psy_results.tex <==
\begin{table*}[!ht]
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
\toprule
\multirow{3}{*}{\textbf{UQ Method}} & \multicolumn{2}{c|}{\textbf{DE}} & \multicolumn{2}{c|}{\textbf{DSM}} & \multicolumn{2}{c|}{\textbf{AL}} & \multicolumn{2}{c|}{\textbf{AD}} & \multicolumn{2}{c}{\textbf{AC}} \\ \cline{2-11}
    & \textbf{RC-AUC} & \begin{tabular}[c]{@{}c@{}} \textbf{RC-AUC} \\ \textbf{50\%}\end{tabular} & \textbf{RC-AUC} & \begin{tabular}[c]{@{}c@{}} \textbf{RC-AUC} \\ \textbf{50\%}\end{tabular} & \textbf{RC-AUC} & \begin{tabular}[c]{@{}c@{}} \textbf{RC-AUC} \\ \textbf{50\%}\end{tabular} & \textbf{RC-AUC} & \begin{tabular}[c]{@{}c@{}} \textbf{RC-AUC} \\ \textbf{50\%}\end{tabular} & \textbf{RC-AUC} & \begin{tabular}[c]{@{}c@{}} \textbf{RC-AUC} \\ \textbf{50\%}\end{tabular} \\
\midrule
SR & 5.2$\pm$2.8 & 3.4$\pm$1.3 & 18.4$\pm$3.2 & 10.4$\pm$0.4 & 19.8$\pm$4.1 & 10.2$\pm$0.8 & 24.9$\pm$1.8 & 11.8$\pm$1.2 & 37.0$\pm$3.5 & 19.7$\pm$0.7 \\
Entropy & 5.2$\pm$2.8 & 3.4$\pm$1.3 & 18.4$\pm$3.2 & 10.4$\pm$0.4 & 19.8$\pm$4.1 & 10.2$\pm$0.8 & 24.9$\pm$1.8 & 11.8$\pm$1.2 & 37.0$\pm$3.5 & 19.7$\pm$0.7 \\
Delta & 5.2$\pm$2.8 & 3.4$\pm$1.3 & 18.4$\pm$3.2 & 10.4$\pm$0.4 & 19.8$\pm$4.1 & 10.2$\pm$0.8 & 24.9$\pm$1.8 & 11.8$\pm$1.2 & 37.0$\pm$3.5 & \underline{19.7$\pm$0.7} \\
Beta & 12.2$\pm$5.7 & 5.4$\pm$1.3 & 19.9$\pm$3.4 & 10.2$\pm$1.0 & 19.5$\pm$2.1 & 10.1$\pm$0.6 & 24.3$\pm$5.0 & 11.1$\pm$1.8 & 41.3$\pm$7.3 & 21.0$\pm$2.1 \\ \midrule
MC (PV) & 8.3$\pm$6.6 & 4.4$\pm$2.7 & 18.2$\pm$3.2 & 10.4$\pm$0.4 & 19.9$\pm$3.9 & \underline{10.0$\pm$1.3} & 23.3$\pm$5.4 & 11.4$\pm$1.8 & 40.9$\pm$4.3 & 20.8$\pm$0.7 \\
MC (SMP) & 8.7$\pm$9.4 & 4.2$\pm$3.4 & \underline{17.9$\pm$2.9} & 10.0$\pm$0.9 & 20.8$\pm$3.4 & 10.2$\pm$0.8 & 23.2$\pm$1.7 & 11.8$\pm$1.0 & 37.7$\pm$3.6 & \underline{19.6$\pm$0.2} \\
MC (BALD) & 9.1$\pm$6.5 & 4.4$\pm$2.6 & 18.0$\pm$3.0 & 10.3$\pm$0.4 & 20.2$\pm$4.2 & \underline{10.0$\pm$1.4} & 23.3$\pm$5.5 & 11.3$\pm$1.7 & 41.4$\pm$4.7 & 20.8$\pm$0.8 \\ \midrule
NUQ ep. & 7.3$\pm$4.4 & 3.9$\pm$2.1 & 18.6$\pm$2.5 & \underline{9.9$\pm$1.4} & \underline{19.2$\pm$3.3} & 10.3$\pm$1.1 & 23.0$\pm$3.7 & 11.1$\pm$1.8 & \underline{36.9$\pm$3.1} & 19.7$\pm$0.9 \\
DDU & 5.1$\pm$3.6 & 3.5$\pm$1.9 & \underline{16.6$\pm$3.9} & \underline{9.6$\pm$1.5} & 20.5$\pm$3.0 & 10.3$\pm$1.0 & \underline{21.6$\pm$5.5} & \underline{11.0$\pm$2.0} & 37.7$\pm$1.7 & \underline{19.6$\pm$0.8} \\
RDE & \underline{4.3$\pm$1.7} & \textbf{3.2$\pm$1.2} & 21.1$\pm$2.3 & 10.6$\pm$1.2 & 22.1$\pm$2.3 & 10.7$\pm$1.0 & \underline{22.0$\pm$4.7} & \underline{11.0$\pm$2.1} & \underline{36.7$\pm$4.5} & 19.9$\pm$0.9 \\
MD & 15.0$\pm$7.1 & 5.9$\pm$2.9 & 23.1$\pm$2.7 & 10.2$\pm$1.3 & \textbf{17.9$\pm$3.1} & \textbf{9.8$\pm$0.8} & \textbf{20.0$\pm$3.9} & \textbf{10.6$\pm$1.7} & 39.3$\pm$5.3 & 20.2$\pm$2.2 \\ \midrule
HUQ-DDU & \underline{4.1$\pm$2.2} & \underline{3.3$\pm$1.3} & 18.0$\pm$3.1 & \underline{9.8$\pm$0.9} & 19.7$\pm$4.1 & 10.2$\pm$0.8 & 23.9$\pm$4.4 & 11.3$\pm$1.8 & \textbf{36.1$\pm$1.2} & \textbf{19.5$\pm$0.7} \\
HUQ2-DDU & \underline{4.3$\pm$2.5} & 3.4$\pm$1.6 & \textbf{16.3$\pm$5.1} & \textbf{9.2$\pm$1.9} & \underline{19.1$\pm$4.2} & \underline{10.0$\pm$0.8} & 22.8$\pm$5.7 & 11.3$\pm$2.0 & 37.4$\pm$3.9 & 20.1$\pm$1.7 \\
HUQ-RDE & 4.3$\pm$1.8 & \underline{3.2$\pm$1.2} & 18.5$\pm$4.0 & 10.4$\pm$0.4 & 21.0$\pm$3.7 & 10.2$\pm$0.8 & 23.4$\pm$3.8 & 11.5$\pm$1.7 & \underline{36.1$\pm$4.5} & 19.8$\pm$0.9 \\
HUQ2-RDE & \textbf{3.9$\pm$1.9} & \underline{3.2$\pm$1.4} & \underline{16.9$\pm$4.1} & 9.9$\pm$0.9 & 19.4$\pm$3.7 & 10.0$\pm$0.7 & 22.5$\pm$5.1 & \underline{11.0$\pm$1.7} & 39.2$\pm$5.2 & 20.5$\pm$1.4 \\
HUQ-MD & 5.7$\pm$2.9 & 3.6$\pm$1.4 & 20.6$\pm$3.7 & 10.6$\pm$0.4 & \underline{19.1$\pm$3.9} & 10.2$\pm$0.8 & \underline{22.5$\pm$3.4} & 11.4$\pm$1.7 & 38.9$\pm$5.7 & 20.0$\pm$2.1 \\
HUQ2-MD & 5.7$\pm$3.6 & 3.5$\pm$1.4 & 18.8$\pm$3.4 & 10.6$\pm$0.5 & 19.5$\pm$3.2 & 10.1$\pm$0.9 & 23.3$\pm$4.9 & 11.4$\pm$1.8 & 40.1$\pm$6.6 & 20.5$\pm$2.7 \\
%HUQ-NUQ & 6.8$\pm$4.2 & 4.0$\pm$2.1 & 18.8$\pm$3.1 & 10.1$\pm$1.0 & 20.6$\pm$3.5 & 10.4$\pm$0.8 & 23.8$\pm$3.8 & 11.3$\pm$1.8 & 37.1$\pm$1.8 & 19.7$\pm$0.9 \\
%HUQ2-NUQ & 6.7$\pm$4.4 & 4.0$\pm$2.4 & 18.7$\pm$3.8 & 10.2$\pm$1.6 & 19.3$\pm$4.1 & 10.1$\pm$0.7 & 24.7$\pm$3.5 & 11.4$\pm$1.9 & 37.5$\pm$3.8 & 20.1$\pm$1.4 \\
\bottomrule
\end{tabular}
}\caption{\label{tab:psy_ue_rubioroberta}Results for the selective classification task for mental disorder detection datasets. The best results for each dataset are shown in bold. We underline top-3 methods after the best.}
\end{table*}

==> tables/psy_results_normalize.tex <==
\begin{table*}[!ht]
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
\toprule
\multirow{3}{*}{\textbf{UQ Method}} & \multicolumn{2}{c|}{\textbf{DE}} & \multicolumn{2}{c|}{\textbf{DSM}} & \multicolumn{2}{c|}{\textbf{AL}} & \multicolumn{2}{c|}{\textbf{AD}} & \multicolumn{2}{c}{\textbf{AC}} \\ \cline{2-11}
    & \textbf{RC-AUC} & \begin{tabular}[c]{@{}c@{}} \textbf{RC-AUC} \\ \textbf{50\%}\end{tabular} & \textbf{RC-AUC} & \begin{tabular}[c]{@{}c@{}} \textbf{RC-AUC} \\ \textbf{50\%}\end{tabular} & \textbf{RC-AUC} & \begin{tabular}[c]{@{}c@{}} \textbf{RC-AUC} \\ \textbf{50\%}\end{tabular} & \textbf{RC-AUC} & \begin{tabular}[c]{@{}c@{}} \textbf{RC-AUC} \\ \textbf{50\%}\end{tabular} & \textbf{RC-AUC} & \begin{tabular}[c]{@{}c@{}} \textbf{RC-AUC} \\ \textbf{50\%}\end{tabular} \\
\midrule
SR & 0.62$\pm$0.26 & 0.53$\pm$0.13 & 0.16$\pm$0.28 & 0.01$\pm$0.19 & 0.06$\pm$0.29 & 0.02$\pm$0.11 & -0.16$\pm$0.28 & -0.29$\pm$0.15 & 0.17$\pm$0.15 & 0.16$\pm$0.16 \\
Entropy & 0.62$\pm$0.26 & 0.53$\pm$0.13 & 0.16$\pm$0.28 & 0.01$\pm$0.19 & 0.06$\pm$0.29 & 0.02$\pm$0.11 & -0.16$\pm$0.28 & -0.29$\pm$0.15 & 0.17$\pm$0.15 & 0.16$\pm$0.16 \\
Delta & 0.62$\pm$0.26 & 0.53$\pm$0.13 & 0.16$\pm$0.28 & 0.01$\pm$0.19 & 0.06$\pm$0.29 & 0.02$\pm$0.11 & -0.16$\pm$0.28 & -0.29$\pm$0.15 & 0.17$\pm$0.15 & 0.16$\pm$0.16 \\
Beta & -0.09$\pm$0.64 & 0.07$\pm$0.42 & 0.07$\pm$0.21 & 0.04$\pm$0.18 & 0.10$\pm$0.17 & 0.02$\pm$0.13 & -0.11$\pm$0.28 & -0.08$\pm$0.26 & 0.03$\pm$0.26 & 0.01$\pm$0.32 \\ \midrule
MC (PV) & 0.39$\pm$0.48 & 0.37$\pm$0.27 & 0.17$\pm$0.29 & 0.01$\pm$0.21 & 0.05$\pm$0.31 & 0.02$\pm$0.34 & -0.04$\pm$0.20 & -0.16$\pm$0.27 & 0.05$\pm$0.14 & 0.02$\pm$0.13 \\
MC (SMP) & 0.42$\pm$0.46 & 0.43$\pm$0.28 & 0.19$\pm$0.26 & 0.08$\pm$0.13 & -0.01$\pm$0.26 & 0.00$\pm$0.11 & -0.04$\pm$0.24 & -0.28$\pm$0.19 & 0.15$\pm$0.17 & \underline{0.17$\pm$0.19} \\
MC (BALD) & 0.31$\pm$0.54 & 0.34$\pm$0.29 & 0.19$\pm$0.27 & 0.01$\pm$0.20 & 0.03$\pm$0.32 & 0.02$\pm$0.37 & -0.03$\pm$0.21 & -0.15$\pm$0.27 & 0.03$\pm$0.13 & 0.02$\pm$0.12 \\
NUQ ep. & 0.49$\pm$0.24 & 0.45$\pm$0.07 & 0.15$\pm$0.18 & 0.09$\pm$0.18 & 0.11$\pm$0.24 & -0.01$\pm$0.25 & -0.02$\pm$0.12 & -0.06$\pm$0.24 & 0.17$\pm$0.16 & 0.16$\pm$0.12 \\ \midrule
DDU & 0.67$\pm$0.18 & 0.53$\pm$0.08 & \underline{0.29$\pm$0.24} & \underline{0.17$\pm$0.18} & 0.03$\pm$0.19 & -0.02$\pm$0.20 & \underline{0.09$\pm$0.24} & \underline{-0.04$\pm$0.25} & 0.15$\pm$0.14 & \underline{0.17$\pm$0.10} \\
RDE & 0.68$\pm$0.20 & \underline{0.55$\pm$0.08} & -0.01$\pm$0.20 & -0.06$\pm$0.14 & -0.08$\pm$0.15 & -0.11$\pm$0.21 & \underline{0.05$\pm$0.15} & -0.06$\pm$0.29 & \underline{0.18$\pm$0.22} & 0.12$\pm$0.10 \\
MD & -0.18$\pm$0.22 & 0.10$\pm$0.11 & -0.14$\pm$0.19 & 0.03$\pm$0.10 & \textbf{0.20$\pm$0.22} & \textbf{0.11$\pm$0.16} & \textbf{0.20$\pm$0.18} & \textbf{0.11$\pm$0.17} & 0.11$\pm$0.09 & 0.09$\pm$0.14 \\ \midrule
HUQ-DDU & \underline{0.73$\pm$0.11} & 0.55$\pm$0.06 & 0.19$\pm$0.24 & \underline{0.13$\pm$0.17} & 0.07$\pm$0.29 & 0.01$\pm$0.12 & -0.09$\pm$0.21 & -0.14$\pm$0.21 & \textbf{0.21$\pm$0.09} & \textbf{0.18$\pm$0.10} \\
HUQ2-DDU & \underline{0.72$\pm$0.11} & 0.54$\pm$0.06 & \textbf{0.30$\pm$0.28} & \textbf{0.24$\pm$0.20} & \underline{0.11$\pm$0.30} & \underline{0.06$\pm$0.09} & 0.00$\pm$0.28 & -0.15$\pm$0.25 & 0.17$\pm$0.06 & 0.10$\pm$0.09 \\
HUQ-RDE & 0.68$\pm$0.21 & \textbf{0.57$\pm$0.07} & 0.16$\pm$0.33 & 0.01$\pm$0.19 & -0.01$\pm$0.25 & 0.02$\pm$0.11 & -0.05$\pm$0.22 & -0.20$\pm$0.20 & \underline{0.20$\pm$0.20} & 0.14$\pm$0.10 \\
HUQ2-RDE & \textbf{0.74$\pm$0.11} & \underline{0.55$\pm$0.06} & \underline{0.26$\pm$0.31} & 0.11$\pm$0.24 & 0.09$\pm$0.27 & 0.04$\pm$0.08 & 0.01$\pm$0.34 & \underline{-0.01$\pm$0.28} & 0.10$\pm$0.22 & 0.05$\pm$0.08 \\
HUQ-MD & 0.58$\pm$0.24 & 0.49$\pm$0.15 & 0.02$\pm$0.31 & -0.04$\pm$0.22 & \underline{0.11$\pm$0.26} & 0.01$\pm$0.10 & 0.02$\pm$0.26 & -0.17$\pm$0.23 & 0.12$\pm$0.09 & 0.11$\pm$0.14 \\
HUQ2-MD & 0.60$\pm$0.23 & 0.50$\pm$0.15 & 0.13$\pm$0.28 & -0.03$\pm$0.16 & 0.09$\pm$0.21 & 0.04$\pm$0.17 & -0.04$\pm$0.31 & -0.16$\pm$0.28 & 0.08$\pm$0.16 & 0.05$\pm$0.22 \\
%HUQ-NUQ & 0.51$\pm$0.27 & 0.44$\pm$0.11 & 0.14$\pm$0.25 & 0.06$\pm$0.15 & 0.01$\pm$0.25 & -0.03$\pm$0.13 & -0.08$\pm$0.17 & -0.13$\pm$0.20 & 0.17$\pm$0.10 & 0.15$\pm$0.10 \\
%HUQ2-NUQ & 0.53$\pm$0.23 & 0.44$\pm$0.13 & 0.14$\pm$0.23 & 0.03$\pm$0.12 & 0.10$\pm$0.29 & \underline{0.04$\pm$0.11} & -0.14$\pm$0.11 & -0.18$\pm$0.24 & 0.16$\pm$0.11 & 0.11$\pm$0.09 \\
\bottomrule
\end{tabular}
}\caption{\label{tab:psy_ue_rubioroberta}Results for the selective classification task for mental disorder detection datasets. The best results for each dataset are shown in bold. We underline top-3 methods after the best.}
\end{table*}

==> tables/results.tex <==
\begin{table*}[!ht] \resizebox{\textwidth}{!}{\begin{tabular}{l|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{\textbf{UE Method}} & \multicolumn{2}{c|}{\textbf{MIMIC Mortality}} & \multicolumn{2}{c|}{\textbf{OV Dataset MCP}} & \multicolumn{2}{c}{\textbf{MIMIC MCP}} \\ \cline{2-7}
    & \textbf{RC-AUC} & \textbf{RC-AUC 50\%} & \textbf{RC-AUC} & \textbf{RC-AUC 50\%} & \textbf{FR-AUC} & \textbf{FR-AUC 50\%} \\
\midrule
% SR & 3340.4$\pm$147.7 & 2268.3$\pm$66.6 & 3654.0 & 2315.7 & 11.1$\pm$2.6 & 26.5$\pm$1.6 \\
% \midrule
% MC (PV) & 2607.5$\pm$47.9 & \textbf{1961.4$\pm$19.1} & 3727.1 & 2430.1 & -17.4$\pm$1.5 & -1.3$\pm$1.6 \\
% MC (SMP) & 2727.5$\pm$56.9 & \underline{1992.2$\pm$20.7} & \underline{3548.1} & \underline{2278.1} & -27.3$\pm$2.4 & -29.9$\pm$2.5 \\
% MC (BALD) & 2582.2$\pm$44.1 & \underline{1970.8$\pm$20.3} & 3691.6 & 2381.9 & -20.5$\pm$1.8 & -14.3$\pm$2.9 \\
% \midrule
% NUQ & 2734.6$\pm$55.6 & 2103.2$\pm$45.6 & 4757.5 & 2652.3 & -3.7$\pm$17.2 & 1.5$\pm$13.7 \\
% DDU & 3782.1$\pm$166.8 & 2249.3$\pm$53.1 & 5100.0 & 2702.7 & 16.0$\pm$2.4 & 27.4$\pm$2.2 \\
% RDE & 2717.8$\pm$106.2 & 2088.1$\pm$26.4 & 4296.3 & 2539.8 & 2.8$\pm$0.9 & 12.3$\pm$1.7 \\
% MD & 3697.7$\pm$171.3 & 2292.7$\pm$55.4 & 5655.3 & 2756.1 & 21.9$\pm$3.8 & 28.9$\pm$2.8 \\
% \midrule
% HUQ-DDU & \underline{2549.0$\pm$54.9} & 2080.2$\pm$40.0 & \underline{3647.8} & \underline{2313.2} & 27.0$\pm$2.2 & 32.9$\pm$1.0 \\
% HUQ2-DDU & \underline{2425.4$\pm$31.8} & 2025.6$\pm$28.7 & 5100.0 & 2702.7 & \underline{\textbf{29.0$\pm$1.4}} & \underline{\textbf{37.3$\pm$0.3}} \\
% HUQ-RDE & 2685.2$\pm$98.8 & 2086.2$\pm$26.1 & \textbf{3386.1} & \textbf{2260.8} & 12.6$\pm$1.7 & 27.1$\pm$1.5 \\
% HUQ2-RDE & 2661.2$\pm$101.8 & 2082.9$\pm$24.7 & \underline{3590.5} & \underline{2279.3} & 11.8$\pm$5.3 & 23.5$\pm$6.4 \\
% HUQ-MD & \underline{2550.3$\pm$54.2} & 2082.0$\pm$38.5 & 5655.3 & 2756.1 & \underline{27.5$\pm$1.6} & \underline{33.1$\pm$1.3} \\
% HUQ2-MD & \textbf{2421.8$\pm$32.9} & \underline{2023.4$\pm$25.4} & 3653.2 & 2317.8 & \underline{27.9$\pm$1.4} & \underline{36.3$\pm$1.3} \\
SR & 3340.4$\pm$147.7 & 2268.3$\pm$66.6 & 3654.0 & 2315.7 & 10.5$\pm$0.6 & 25.3$\pm$1.2 \\
Entropy & 11308.5$\pm$124.0 & 4077.2$\pm$56.9 & 3690.2 & 2343.1 & 11.6$\pm$0.8 & 17.2$\pm$0.7 \\
Delta & 11308.5$\pm$124.0 & 4077.2$\pm$56.9 & 3683.2 & 2341.6 & 11.6$\pm$0.4 & 14.4$\pm$0.5 \\
Beta & 3448.4$\pm$165.1 & 2304.6$\pm$43.1 & 3654.2 & 2315.9 & -30.3$\pm$0.8 & -6.6$\pm$0.3 \\\midrule
MC (PV) & 2607.5$\pm$47.9 & \textbf{1961.4$\pm$19.1} & 3727.1 & 2430.1 & -22.2$\pm$1.5 & -4.3$\pm$1.5 \\
MC (SMP) & 2727.5$\pm$56.9 & \underline{1992.2$\pm$20.7} & \underline{3548.1} & \underline{2278.1} & -25.5$\pm$0.6 & -22.9$\pm$1.4 \\
MC (BALD) & 2582.2$\pm$44.1 & \underline{1970.8$\pm$20.3} & 3691.6 & 2381.9 & -21.4$\pm$1.3 & -11.8$\pm$1.7 \\\midrule
NUQ ep. & 2682.4$\pm$216.9 & 2115.9$\pm$108.5 & 4818.9 & 2651.1 & 11.0$\pm$0.7 & 14.2$\pm$0.4 \\
DDU & 3782.1$\pm$166.8 & 2249.3$\pm$53.1 & 5100.0 & 2702.7 & 20.2$\pm$2.5 & 24.3$\pm$1.3 \\
RDE & 2717.8$\pm$106.2 & 2088.1$\pm$26.4 & 4308.9 & 2544.9 & 6.4$\pm$0.7 & 15.0$\pm$0.4 \\
MD & 3697.7$\pm$171.3 & 2292.7$\pm$55.4 & 5655.3 & 2756.1 & 24.1$\pm$2.4 & 26.4$\pm$1.4 \\\midrule
HUQ-DDU & \underline{2549.0$\pm$54.9} & 2080.2$\pm$40.0 & \underline{3647.8} & \underline{2313.2} & \underline{26.8$\pm$1.0} & 30.2$\pm$1.1 \\
HUQ2-DDU & \underline{2425.4$\pm$31.8} & 2025.6$\pm$28.7 & 5100.0 & 2702.7 & \underline{\textbf{27.5$\pm$0.6}} & \underline{34.4$\pm$1.1} \\
HUQ-RDE & 2685.2$\pm$98.8 & 2086.2$\pm$26.1 & \textbf{3382.9} & \textbf{2261.5} & 11.7$\pm$0.5 & 25.6$\pm$0.8 \\
HUQ2-RDE & 2661.2$\pm$101.8 & 2082.9$\pm$24.7 & \underline{3602.3} & \underline{2280.3} & 11.4$\pm$2.9 & 24.0$\pm$5.1 \\
HUQ-MD & \underline{2550.3$\pm$54.2} & 2082.0$\pm$38.5 & 5655.3 & 2756.1 & 26.4$\pm$1.6 & \underline{30.6$\pm$1.3} \\
HUQ2-MD & \textbf{2421.8$\pm$32.9} & \underline{2023.4$\pm$25.4} & 3653.2 & 2317.8 & \underline{27.0$\pm$1.1} & \underline{\textbf{34.5$\pm$1.1}} \\
\bottomrule
\end{tabular}
}\caption{\label{tab:mimic} Results for the selective classification task for the considered datasets. For the MIMIC mortality detection and OV datasets, we use RC-AUC$\downarrow$ and RC-AUC$\downarrow$ on the first 50\% of the curve metrics. For the MIMIC medical code prediction task, we use the area under the F1-micro rejection curve (FR-AUC$\uparrow$) on the full curve and the first 50\% of the curve. The best results for each dataset are shown in bold. We underline top-3 methods after the best.}\end{table*}

==> tables/results_normalized_all.tex <==
\begin{table*}[!ht]
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{\textbf{UE Method}} & \multicolumn{2}{c|}{\textbf{MIMIC Mortality}} & \multicolumn{2}{c|}{\textbf{OV Dataset MCP}} & \multicolumn{2}{c}{\textbf{MIMIC MCP}} \\ \cline{2-7}
    & \textbf{RC-AUC} & \textbf{RC-AUC 50\%} & \textbf{RC-AUC} & \textbf{RC-AUC 50\%} & \textbf{FR-AUC} & \textbf{FR-AUC 50\%} \\
\midrule
SR & 0.55$\pm$0.01 & 0.38$\pm$0.01 & 0.48 & 0.4 & 0.10$\pm$0.01 & 0.25$\pm$0.01 \\
Entropy & -0.75$\pm$0.02 & -0.27$\pm$0.01 & 0.47 & 0.37 & 0.12$\pm$0.01 & 0.17$\pm$0.01 \\
Delta & -0.75$\pm$0.02 & -0.27$\pm$0.01 & 0.47 & 0.38 & 0.12$\pm$0.00 & 0.14$\pm$0.01 \\
Beta & 0.53$\pm$0.03 & 0.37$\pm$0.02 & 0.48 & 0.4 & -0.30$\pm$0.01 & -0.07$\pm$0.00 \\\midrule
MC (PV) & 0.66$\pm$0.01 & \textbf{0.49$\pm$0.01} & 0.46 & 0.28 & -0.22$\pm$0.01 & -0.04$\pm$0.01 \\
MC (SMP) & 0.64$\pm$0.01 & \underline{0.48$\pm$0.01} & \underline{0.51} & \underline{0.44} & -0.26$\pm$0.01 & -0.23$\pm$0.01 \\
MC (BALD) & 0.67$\pm$0.01 & \underline{0.49$\pm$0.01} & 0.47 & 0.33 & -0.21$\pm$0.01 & -0.12$\pm$0.02 \\\midrule
NUQ ep. & 0.65$\pm$0.03 & 0.44$\pm$0.03 & 0.18 & 0.05 & 0.11$\pm$0.01 & 0.14$\pm$0.00 \\
DDU & 0.47$\pm$0.03 & 0.39$\pm$0.02 & 0.08 & -0.0 & 0.20$\pm$0.03 & 0.24$\pm$0.01 \\
RDE & 0.65$\pm$0.02 & 0.45$\pm$0.02 & 0.3 & 0.17 & 0.06$\pm$0.01 & 0.15$\pm$0.00 \\
MD & 0.49$\pm$0.03 & 0.37$\pm$0.02 & -0.07 & -0.06 & 0.24$\pm$0.02 & 0.26$\pm$0.01 \\\midrule
HUQ-DDU & \underline{0.67$\pm$0.01} & 0.45$\pm$0.01 & \underline{0.48} & \underline{0.41} & \underline{0.27$\pm$0.01} & \underline{0.30$\pm$0.01} \\
HUQ2-DDU & \underline{0.69$\pm$0.01} & 0.47$\pm$0.01 & 0.08 & -0.0 & \textbf{0.28$\pm$0.01} & \underline{0.34$\pm$0.01} \\
HUQ-RDE & 0.65$\pm$0.02 & 0.45$\pm$0.01 & \textbf{0.56} & \textbf{0.47} & 0.12$\pm$0.01 & 0.26$\pm$0.01 \\
HUQ2-RDE & 0.66$\pm$0.02 & 0.45$\pm$0.02 & \underline{0.5} & \underline{0.44} & 0.11$\pm$0.03 & 0.24$\pm$0.05 \\
HUQ-MD & \underline{0.67$\pm$0.01} & 0.45$\pm$0.01 & -0.07 & -0.06 & \underline{0.26$\pm$0.02} & \underline{0.31$\pm$0.01} \\
HUQ2-MD & \textbf{0.69$\pm$0.01} & \underline{0.47$\pm$0.01} & 0.48 & 0.4 & \underline{0.27$\pm$0.01} & \textbf{0.34$\pm$0.01} \\
\bottomrule
\end{tabular}
}\caption{\label{tab:mimic} Results for the selective classification task for MIMIC mortality, OV, and MIMIC MCP  datasets. For the MIMIC mortality detection and OV datasets, we use normalized RC-AUC$\uparrow$ and normalized RC-AUC$\uparrow$ on the first 50\% of the curve metrics. For the MIMIC medical code prediction task, we use the area under the F1-micro rejection curve (FR-AUC$\uparrow$) on the full curve and the first 50\% of the curve. The best results for each dataset are shown in bold. We underline top-3 methods after the best.}
\end{table*}
